Kara: A System for Visualising and Visual Editing of Interpretations for Answer-Set Programs

In answer-set programming (ASP), the solutions of a problem are encoded in dedicated models, called answer sets, of a logical theory. These answer sets are computed from the program that represents the theory by means of an ASP solver and returned to the user as sets of ground first-order literals. As this type of representation is often cumbersome for the user to interpret, tools like ASPVIZ and IDPDraw were developed that allow for visualising answer sets. The tool Kara, introduced in this paper, follows these approaches, using ASP itself as a language for defining visualisations of interpretations. Unlike existing tools that position graphic primitives according to static coordinates only, Kara allows for more high-level specifications, supporting graph structures, grids, and relative positioning of graphical elements. Moreover, generalising the functionality of previous tools, Kara provides modifiable visualisations such that interpretations can be manipulated by graphically editing their visualisations. This is realised by resorting to abductive reasoning techniques. Kara is part of SeaLion, a forthcoming integrated development environment (IDE) for ASP.

==> command.tex <==
% !TEX root =  paper.tex
\newcommand{\naf}{\ensuremath{\mathrm{not}}\xspace}
\newcommand{\sneg}[1]{\ensuremath{\neg#1}\xspace}
\newcommand{\compl}[1]{\ensuremath{\bar{#1}}}

\newcommand{\atomp}[1]{\ensuremath{\mathit{#1}\xspace}}
\newcommand{\atom}[2]{\ensuremath{\mathtt{#1}{\rm(}\mathtt{#2}{\rm)}\xspace}}
\renewcommand{\atom}[2]{\ensuremath{\mathit{#1}{(}{#2}{)}\xspace}}




\newcommand{\gringo}{\texttt{Gringo}\xspace}
\newcommand{\aspviz}{\texttt{ASPVIZ}\xspace}
\newcommand{\idpdraw}{\texttt{IDPDraw}\xspace}
\newcommand{\clasp}{\textsc{Clasp}\xspace}
\newcommand{\dlv}{\texttt{DLV}\xspace}
\newcommand{\nomore}{\texttt{noMoRe}\xspace}
\newcommand{\inter}{\ensuremath{I}\xspace}
\newcommand{\ninter}{\ensuremath{N}\xspace}
\newcommand{\deltaR}{\ensuremath{{\mathit{R}_\Delta}}\xspace}
\newcommand{\deltaI}{\ensuremath{{\mathit{I}_\Delta}}\xspace}
\newcommand{\loopS}{\ensuremath{\Gamma}\xspace}
\newcommand{\opsym}[1]{\ensuremath{\Upsilon_{#1}}\xspace}
\newcommand{\op}[2]{\ensuremath{\opsym{#1}({#2})}\xspace}
%\newcommand{\statei}[1]{\ensuremath{\mathit{I}_{#1}}\xspace}
\newcommand{\statei}[1]{\ensuremath{\mathit{I}({#1})}\xspace}
\renewcommand{\statei}[1]{\ensuremath{\mathit{Int}[{#1}]}\xspace}
\newcommand{\stater}[1]{\ensuremath{\mathit{R}_{#1}}\xspace}
\newcommand{\cset}{\ensuremath{C}\xspace}
\newcommand{\state}{\ensuremath{S}\xspace}
\newcommand{\facts}{\ensuremath{F}\xspace}
\newcommand{\computation}{\ensuremath{\mathrm{C}}\xspace}
\newcommand{\blockedLiterals}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\applrules}{\ensuremath{R}\xspace}
\newcommand{\activatedRules}[2]{\ensuremath{\mathit{AR}_{#2}(#1)}\xspace}

\newcommand{\sealion}{\texttt{SeaLion}\xspace}
\newcommand{\kara}{\texttt{Kara}\xspace}

\newcommand{\intconstraints}[1]{\ensuremath{\mathit{Con}_{#1}}\xspace}

\newcommand{\activerules}[2]{\ensuremath{\mathit{Act}^{#1}({#2})}\xspace}

\newcommand{\forbidden}{\ensuremath{\mathit{forbidden}}\xspace}
\newcommand{\currentSupport}[1]{\ensuremath{\mathit{Sup}[{#1}]}\xspace}
\newcommand{\pool}{\ensuremath{\mathit{pool}}\xspace}
\newcommand{\hcpool}{\ensuremath{\mathit{pool^{HC}}}\xspace}
\newcommand{\constraintset}{\ensuremath{\mathit{Con}}\xspace}
\newcommand{\hclits}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\Pol}{{\rm P}\xspace}
\newcommand{\PNP}{\Pol^{\rm NP}\xspace}
\newcommand{\NP}{\mbox{\rm NP}\xspace}
\newcommand{\NPNP}{\NP^{\rm NP}\xspace}
\newcommand{\CONP}{\mbox{\rm coNP}\xspace}
\newcommand{\coNP}{\mbox{\rm coNP}\xspace}
\newcommand{\SigmaP}[1]{\ensuremath{{\Sigma}_{#1}^{P}}\xspace}
\newcommand{\PiP}[1]{\ensuremath{{\Pi}_{#1}^{P}}\xspace}
\newcommand{\DeltaP}[1]{\ensuremath{{\Delta}_{#1}^{P}}\xspace}

\newcommand{\lang}{\ensuremath{\mathcal{L}}\xspace}

\newcommand{\alphabet}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\visalphabet}{\ensuremath{\mathcal{A}_V}\xspace}

\newcommand{\vispred}{\ensuremath{\mathcal{P}_v}\xspace}
\newcommand{\abdpred}{\ensuremath{\mathcal{P}_a}\xspace}
\newcommand{\intpred}{\ensuremath{\mathcal{P}_i}\xspace}
\newcommand{\abddom}{\ensuremath{\mathcal{D}_a}\xspace}

\newcommand{\la}{\ensuremath{\leftarrow}\xspace}
\newcommand{\ra}{\ensuremath{\rightarrow}\xspace}
\newcommand{\at}[1]{\ensuremath{\mathit{At}(#1)}\xspace}

\newcommand{\subst}{\ensuremath{\vartheta}\xspace}

\newcommand{\succeeds}[1]{\ensuremath{\succ_{#1}}\xspace}
\renewcommand{\succeeds}[1]{\ensuremath{\prec_{#1}}\xspace}
\newcommand{\result}[1]{\ensuremath{\mathit{res}({#1})}\xspace}

\newcommand{\be}{\begin{compactenum}}
\newcommand{\ee}{\end{compactenum}}
\newcommand{\bi}{\begin{compactitem}}
\newcommand{\ei}{\end{compactitem}}

\newcommand{\AS}[1]{\ensuremath{\mathit{AS}(#1)}\xspace}
\newcommand{\SM}[1]{\AS{#1}}

\newcommand{\naturals}[0]{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\vhack}{\vspace{-8pt}}
\newcommand{\vhackafter}{\vspace{-5.5pt}}
\renewcommand{\vhack}{}
\renewcommand{\vhackafter}{}
\newcommand{\lit}[1]{\ensuremath{\mathit{L}(#1)}\xspace}


\newcommand{\hcfuncsym}[2]{\ensuremath{f_{#1,#2}}\xspace}
\newcommand{\hcfunc}[3]{\ensuremath{\hcfuncsym{#1}{#2}({#3})}\xspace}

\newcommand{\viz}[0]{viz.\xspace}
\newcommand{\wrt}[0]{with respect to\xspace}
%\newcommand{\wrt}[0]{w.r.t.\xspace}
\newcommand{\iec}[0]{i.e.,\xspace}
\newcommand{\Iec}[0]{I.e.,\xspace}
\newcommand{\egc}[0]{e.g.,\xspace}
\newcommand{\eg}[0]{e.g.\xspace}
\newcommand{\resp}[0]{resp.,\xspace}
\newcommand{\nop}[1]{}
\newcommand{\body}[1]{\ensuremath{\mathrm{B(}{#1}\mathrm{)}}\xspace}
\newcommand{\head}[1]{\ensuremath{\mathrm{H(}{#1}\mathrm{)}}\xspace}
\newcommand{\pbody}[1]{\ensuremath{\mathrm{{B^+}(}{#1}\mathrm{)}}\xspace}
\newcommand{\nbody}[1]{\ensuremath{\mathrm{{B^-}(}{#1}\mathrm{)}}\xspace}
\newcommand{\gr}[1]{\ensuremath{\mathit{gr(}{#1}\mathit{)}}\xspace}
\newcommand{\tupel}[1]{\ensuremath{\langle {#1} \rangle}\xspace}
\newcommand{\set}[1]{\ensuremath{\{{#1}\}}\xspace}
\newcommand{\abs}[1]{\ensuremath{|{#1}|}\xspace}
\newcommand{\selfsupp}[0]{self-supporting\xspace}
\newcommand{\stable}[0]{stable\xspace}


\newcommand{\trans}[2]{\ensuremath{\lambda{\rm(}{#1},{#2}{\rm)}}}
\newcommand{\guesspart}[1]{\ensuremath{\mathit{guess}{\rm(}{#1}{\rm)}}}
\renewcommand{\guesspart}[1]{\ensuremath{\mathsf{guess}{\rm(}{#1}{\rm)}}}
\newcommand{\checkpart}[1]{\ensuremath{\mathit{check}{\rm(}{#1}{\rm)}}}
\renewcommand{\checkpart}[1]{\ensuremath{\mathsf{check}{\rm(}{#1}{\rm)}}}
\newcommand{\var}[1]{\ensuremath{\mathit{VAR}{\rm(}{#1}{\rm)}}}
\newcommand{\dompart}[2]{\ensuremath{\mathit{dom}{\rm(}{#1},{#2}{\rm)}}}
\renewcommand{\dompart}[2]{\ensuremath{\mathsf{dom}{\rm(}{#1},{#2}{\rm)}}}

\newcommand{\ruleimp}{\mathtt{{:-}}}
\renewcommand{\ruleimp}{:\!- \ }

\newcommand{\nonrecdomo}[0]{\ensuremath{\mathtt{nonRecDom}}}
\renewcommand{\nonrecdomo}[0]{\ensuremath{\mathit{nonRecDom}}}
\newcommand{\nonrecdom}[1]{\ensuremath{\nonrecdomo(#1)}}
\newcommand{\domo}[0]{\ensuremath{\mathtt{dom}}}
\renewcommand{\domo}[0]{\ensuremath{\mathit{dom}}}
\newcommand{\dom}[1]{\ensuremath{\domo(#1)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

